GG-LLM: Geometrically Grounding Large Language Models for Zero-shot Human Activity Forecasting in Human-Aware Task Planning

A robot in a human-centric environment needs to account for the human's intent and future motion in its task and motion planning to ensure safe and effective operation. This requires symbolic reasoning about probable future actions and the ability to tie these actions to specific locations in the physical environment. While one can train behavioral models capable of predicting human motion from past activities, this approach requires large amounts of data to achieve acceptable long-horizon predictions. More importantly, the resulting models are constrained to specific data formats and modalities. Moreover, connecting predictions from such models to the environment at hand to ensure the applicability of these predictions is an unsolved problem. We present a system that utilizes a Large Language Model (LLM) to infer a human's next actions from a range of modalities without fine-tuning. A novel aspect of our system that is critical to robotics applications is that it links the predicted actions to specific locations in a semantic map of the environment. Our method leverages the fact that LLMs, trained on a vast corpus of text describing typical human behaviors, encode substantial world knowledge, including probable sequences of human actions and activities. We demonstrate how these localized activity predictions can be incorporated in a human-aware task planner for an assistive robot to reduce the occurrences of undesirable human-robot interactions by 29.2% on average.

==> old_notes/old_notes.tex <==

\section{Problem formulation}
A robot agent operates in a human-occupied environment. The agent aims to complete a set of tasks while minimizing disturbance to the humans, where our understanding of a disturbance includes both possibly unsafe (i.e., collision with the human) and inconvenient robot behaviors, such as the robot being visible or audible to the human, or standing in their way.

\section{Room sweeping task}
We demonstrate the utilit

We construct a representative assistive robot task in which a robot is tasked to move around in an indoor environment with $N$ rooms $\{R_1,R_2,...,R_N\}$. The robot moves from one room to the other, spending $T_{max}$ time steps in each room before moving onto the next room. This task is motivated by, and closely related to, common assistive robot applications, including home cleaning, tidying up, collecting items required for xx, or routine inspection and security in warehouses, offices, ...


world $\mathcal{W}$ containing a set of object instances $I$, each of which can have multiple occurrences, resulting in a bag of objects that is an ordered pair $(I,m)$ where $m: I\to\mathbb{Z}^+$ maps each instance to its (positive integer) multiplicity. 


state of the agent at time $t$: $s_t$, includes integrator of time 

state of the human: position coords; 

transition functions:

baseline policy: random walk; transition to random room as soon as time spent in current room reaches $T_{max}$, reset integrator

baseline policy: random walk into any room BUT the one currently occupied by the human

baseline oracle policy: knows exactly where the human will be over the next $T_{max}$ steps and randomly pick one of the rooms for which the time of the human in that room is minimal

LLM policy 1: assign scores $sc_i$ to each instance as the completion. sum scores over instances per room to get the probability they are going to said room. pick the room with the lowest score.

LLM policy 2: same as above but remove the current room of the human from the possible options to transition to. 

sequence of states under policy $\pi$: $S_t=o$ xx how to write? check RL works

metric: summation over all time of dot product of human occupation and robot occupation


\section{A fresh start}
Possible goals: all objects extracted from the environment (roughly 100-200)

We want to predict 

challenges with MCQA: cloze prompt vs providing and asking it to predict an answer
- asking to pick an answer from (A, B, C, D): people have observed bias
- with more potential options, i am sure it will fail eventually, but I havent tested this

Challenges with observations: 
detergent vs laundry detergent
Challenges/questions with scoring completions: completion length, "is" vs "ia"; typos; what about synonyms?

another possible approach for length normalization: take L-th root if length L

step-by-step:
\begin{enumerate}
    \item Extract possible goal locations $G^i=(x^i,y^i,\mathbf{g}^i)$ with coordinates $(x^i,y^i)$ and text description $\mathbf{g}^i$ 
    \item Compute score $s^i$ for each goal completions  $\mathbf{g}^i$ ($\sum_i s_i=1$)
    
\end{enumerate}

metrics accuracy, callibratedness, speed



% \setstretch{1.5} % set to \setstretch{1} (or remove) for single space
\section{Overview}
\begin{enumerate}
    \item Create semantic map $\mathcal{M}$ of the environment $E$
    \item Extract possible goal locations from $\mathcal{M}$ (this could also just return all goal locations)
    \item Observe the human and the environment and create a narration $\mathbf{N}$ from these observations
    \item Get the likelihood for each possible goal location with the method outlined in Section~\ref{s:appA}
    \item Estimate likely human goals from trajectory history and combine this with LLM-based goal likelihood
    \item Derive likely human trajectories based on inferred human goal
    \item Robot helper: plan to solve its task while minimizing friction/interactions with the human (integration with RAMP team)
\end{enumerate}


\section{Grounding human goal predictions in reality}

\textbf{Given:} 

\begin{itemize}
    \item  A representation of the environment $E$ in form of a semantic map $\mathcal{M} \in \mathbb{R}^{L\times W \times C}$, where $L$,$W$ are the length and width of the grid representing the top-down floor plan, and $C$ is the dimension of the feature vector encoding semantic information for each grid cell of the floor plan. $\mathcal{M}$ can be a floor plan with semantic information, a dense visual language map (or \textit{VLMap} as presented in \cite{huang2022visual}), or a sparse map with localized language labels from key frames / key points only. Note that we could also use voxels to represent the semantic map by adding an additional dimension.
    \item A narration $\mathbf{N}$ about the human, the time, and the state of the apartment. $\mathbf{N}$ is a sequence of tokens that contains a description of the apartment state, and narration of the human and what they are holding/doing.
    \item A binding token sequence $\mathbf{B}$, for example "The human is walking towards the " (note: could try to achieve robustness by averaging over various binding sequences, or design an experiment that evaluates the effect of different instantiations for $\mathbf{B}$)
\end{itemize}

\textbf{Find:}
The likelihood $\mathcal{G}_{LMM} \in \mathbb{R}^{L \times W}$ that a cell in ${L \times W}$ is the human's goal.


\subsection{Approach A}
\label{s:appA}
From the semantic map $\mathcal{M}$ extract possible goal locations $G^i=(x^i,y^i,\mathbf{g}^i)$ with coordinates $(x^i,y^i)$ and text description $\mathbf{g}^i$ (for example, $\mathbf{g}^i$ may be "the kitchen", "the laundry machine in the laundry room", or "the dish washer in the kitchen"). These text descriptions consists of a sequence of $n$ tokens $\mathbf{g^i}=g^i_1, . . . , g^i_{n}$. In the following notation, we drop the goal index $i$ to simplify notation.

Let $p_M(z_{n+1} | z_1, . . . , z_n)$ be the probability that the language model $M$ assigns to token $z_{n+1}$ as a continuation for the sequence $z_1, . . . , z_n$. For many models, including the LLaMA architecture, we can compute $p_M$ as follows: 
$$
p_M(z_{n+1} | z_1, . . . , z_n)=\text{softmax}(l_M | z_1, . . . , z_n)$$ where $l_M$ are the logits of the model. The logits can be obtained with a simple forward pass of $M$ as $l_M=f_M(z_1, . . . , z_n)$. Clear exemplary code for computing $p_M$ for the LLaMA model using the Lighting-AI framework can be found at \url{https://github.com/Lightning-AI/lit-llama/blob/main/generate.py}.

Given narration $\mathbf{N}$, binding sequence $\mathbf{B}$, and a sequence of weights $w_j$, the weighted cross entropy loss for $M$ over the token sequence $\mathbf{g} = g_1, . . . , g_n$ as a completion of $\mathbf{N}+\mathbf{B}$ (where $+$ indicates string concatenation) is

$$L(\mathbf{g})=-\sum_{j=1}^n w_j \log p_M(g_j|\mathbf{N}+\mathbf{B}+g_{1:j})$$

We can use this to create a map of likely goals by computing $L(\mathbf{g}=\mathbf{g^i})$ for all $\mathbf{g^i}$ available in our environment.

Alternatively, we can directly compute the probability of a given goal sequence as stated below (note that this may result in higher numerical errors)
$$
P(\mathbf{g}|\mathbf{N}+\mathbf{B})=\prod_{j=1}^n p_M(g_j|\mathbf{N}+\mathbf{B}+g_{1:j})
$$

\subsection{Approach B}
This approach requires a shared embedding between a visual-semantic representation of the map (i.e., VLMap) and the language model with identical tokenization. 

Compute a group of $m$ most likely completions to the prompt $\mathbf{N}+\mathbf{B}$ (we will need to think about how to encourage that the suggested completions are diverse). search for peaks in similarity between most likely prompt completions and the semantic map (through dot product)

\subsection{Approach C}

Loop through the semantic map (not necessarily at smallest possible resolution of course); for each semantic feature $g$ in the map, compute  $L(\mathbf{g})$ as defined above.


\section{Combination with motion-based prediction}
Finally, we should combine the LLM-predicted goal and with predictions inferred from the past trajectory with a motion-based approach.  


\newpage
\onecolumn

\section{Table with results}
\begin{tabular}{llllllllll}
\toprule
 & Oracle & Random & LeastItems & LeastOcc & LLM & Random+A & LeastItems+A & LeastOcc+A & LLM+A \\
\midrule
c0, 0, T=25 & 7.0±8.1 & 164.6±50.2 & 182.4±8.0 & 134.4±8.0 & 65.9±8.1 & 36.8±20.7 & 8.9±8.0 & 30.4±8.0 & 22.6±14.5 \\
c0, 0, T=50 & 13.7±13.3 & 160.5±62.7 & 189.3±13.3 & 116.4±13.3 & 72.7±13.3 & 65.6±29.3 & 40.8±13.3 & 58.8±13.4 & 58.1±20.0 \\
c0, 0, T=100 & 45.7±34.1 & 145.3±66.2 & 203.2±34.0 & 97.7±34.0 & 86.6±34.0 & 110.0±48.9 & 54.7±34.0 & 112.7±34.1 & 86.6±34.0 \\
c0, 4, T=25 & 7.0±11.2 & 146.2±45.4 & 75.4±11.3 & 75.4±11.3 & 96.5±11.3 & 42.7±21.2 & 20.0±11.2 & 20.0±11.2 & 62.4±11.2 \\
c0, 4, T=50 & 13.5±15.5 & 139.9±61.8 & 69.0±15.5 & 69.0±15.5 & 111.5±15.5 & 65.6±34.6 & 13.5±15.5 & 13.5±15.5 & 61.5±15.5 \\
c0, 4, T=100 & 25.8±26.3 & 129.8±68.3 & 31.3±26.3 & 31.3±26.3 & 123.8±26.4 & 123.9±69.4 & 25.8±26.3 & 25.8±26.3 & 123.8±26.4 \\
c0, 5, T=25 & 6.3±10.8 & 167.0±52.2 & 163.7±10.9 & 163.6±11.0 & 37.7±10.8 & 41.5±21.9 & 34.7±10.9 & 39.2±16.3 & 12.7±10.8 \\
c0, 5, T=50 & 12.8±15.6 & 163.4±68.7 & 170.1±15.6 & 145.6±15.7 & 44.1±15.6 & 70.6±40.4 & 66.1±15.6 & 79.1±26.2 & 44.1±15.6 \\
c0, 5, T=100 & 26.6±26.7 & 148.2±75.3 & 184.1±26.7 & 115.5±26.7 & 108.1±26.7 & 109.2±66.0 & 124.1±26.7 & 115.5±26.7 & 108.1±26.7 \\
c1, 0, T=25 & 6.4±10.5 & 165.0±51.9 & 145.6±10.6 & 113.6±10.5 & 114.1±10.6 & 57.3±26.0 & 25.6±15.3 & 23.6±10.5 & 33.8±10.7 \\
c1, 0, T=50 & 12.1±12.5 & 156.7±58.5 & 126.9±12.6 & 119.3±12.5 & 119.9±12.5 & 72.6±29.3 & 18.4±12.6 & 29.3±12.5 & 39.9±12.6 \\
c1, 0, T=100 & 29.4±29.8 & 142.8±65.4 & 88.8±29.9 & 130.8±29.8 & 130.8±29.8 & 112.7±54.3 & 29.9±29.8 & 123.8±29.7 & 111.9±29.9 \\
c1, 4, T=25 & 6.6±6.3 & 134.0±47.2 & 6.6±6.3 & 6.6±6.3 & 6.6±6.3 & 16.7±10.0 & 6.6±6.3 & 6.6±6.3 & 6.6±6.3 \\
c1, 4, T=50 & 12.8±15.2 & 128.7±59.5 & 12.8±15.2 & 12.8±15.2 & 12.8±15.2 & 40.7±26.8 & 12.8±15.2 & 12.8±15.2 & 12.8±15.2 \\
c1, 4, T=100 & 25.1±36.2 & 116.4±62.9 & 25.1±36.2 & 25.1±36.2 & 25.1±36.2 & 72.9±51.7 & 25.1±36.2 & 25.1±36.2 & 25.1±36.2 \\
c1, 5, T=25 & 6.5±10.8 & 146.4±48.5 & 165.1±10.9 & 108.2±11.0 & 108.2±11.0 & 36.4±19.9 & 35.2±15.6 & 23.6±10.9 & 28.5±14.6 \\
c1, 5, T=50 & 13.1±12.7 & 140.5±57.1 & 162.4±12.7 & 115.0±12.9 & 115.0±12.9 & 67.4±37.1 & 76.9±26.7 & 55.5±12.8 & 70.1±12.8 \\
c1, 5, T=100 & 30.3±14.9 & 127.6±50.0 & 91.7±15.0 & 127.3±15.0 & 127.3±15.0 & 83.4±35.9 & 81.7±14.9 & 67.8±14.9 & 82.3±14.9 \\
c2, 0, T=25 & 6.7±10.8 & 345.4±78.0 & 248.7±10.8 & 399.2±11.1 & 174.2±11.0 & 64.5±27.6 & 19.6±15.8 & 40.4±10.9 & 69.6±19.3 \\
c2, 0, T=50 & 12.5±21.6 & 335.1±92.5 & 254.8±21.6 & 405.4±21.5 & 155.3±21.9 & 129.4±48.3 & 38.3±21.5 & 86.9±21.6 & 145.3±21.8 \\
c2, 0, T=100 & 25.8±27.5 & 321.7±122.4 & 268.1±27.6 & 395.6±27.6 & 191.8±27.7 & 184.2±80.2 & 101.6±27.5 & 147.5±27.6 & 203.7±27.5 \\
c2, 4, T=25 & 7.7±11.3 & 330.0±75.0 & 58.9±11.3 & 58.9±11.3 & 105.5±11.4 & 67.3±27.8 & 13.9±11.3 & 13.9±11.3 & 45.5±11.3 \\
c2, 4, T=50 & 14.3±22.4 & 325.4±97.2 & 40.9±22.4 & 40.9±22.4 & 110.4±22.4 & 138.9±57.6 & 40.9±22.4 & 40.9±22.4 & 50.4±22.4 \\
c2, 4, T=100 & 42.6±44.8 & 314.1±127.8 & 27.8±44.8 & 27.8±44.8 & 106.3±44.9 & 184.9±93.4 & 27.8±44.8 & 27.8±44.8 & 87.3±44.8 \\
c2, 5, T=25 & 6.5±10.8 & 320.9±70.3 & 326.2±10.8 & 416.7±11.0 & 103.5±11.0 & 39.2±22.4 & 21.1±10.9 & 30.8±15.3 & 49.1±16.2 \\
c2, 5, T=50 & 12.5±21.6 & 313.2±99.7 & 332.3±21.6 & 422.8±21.7 & 109.8±21.6 & 62.2±38.2 & 39.3±21.6 & 26.0±21.6 & 51.6±23.1 \\
c2, 5, T=100 & 24.7±43.1 & 308.7±138.9 & 344.6±43.1 & 404.6±43.0 & 152.6±43.2 & 124.5±82.4 & 51.6±43.2 & 87.6±43.0 & 52.6±43.2 \\
\bottomrule
\end{tabular}



\section{Human trajectory forecasting}
 We want to predict the future human trajectory/position for the next $T$ steps. We can either predict the coordinates $s_{t:t+T}$ of the human's Center of Mass (CoM) or predict the likelihood of occupancy for the next $T$ steps on an occupancy grid $\mathcal{O}_{t:t+T} \in \mathbb{R}^{L\times W}$
 
\textbf{Given:} A semantic map $\mathcal{M}$, a map indicating likely human goals $\mathcal{G}$.

\textbf{Find:} The likelihood of occupancy for the next $T$ steps on an occupancy grid $\mathcal{O}_{t:t+T} \in \mathbb{R}^{L\times W}$

\subsection{Approach}
If $\mathcal{M}$ is a dense representation, we can get the 2D traversability map $\mathcal{T}$ from $\mathcal{M}$ by projecting $C$ to one dimension with a binary score that indicates whether the underlying area is traversable or not. Alternatively, we could project $C$ to a continuous traversing cost score that reflects the a priori likelihood of the human to traverse a certain area (e.g., a grid cell containing wall features in $C$ should have a traversability of $0$; tables should result in similarly low traversability; chairs and easily movable obstacles should have a higher traversability; and open space should be easily traversable. 

We can construct an estimate of the human's utility or state-action value function $\hat{Q}(s,a)$ from $\mathcal{G}$ and $\mathcal{T}$.

Then, the trajectory can be obtained under the assumption that the human is an agent taking action $a_t$ with the goal to maximize its utility. A perfectly rational agent would take the action $a_*=\arg\max_a Q(s,a)$. Following a noisy-rationality decision model (e.g., \cite{ziebart2008maximum}, but also applied and discussed in depth in \cite{fisac2018probabilistically}) instead of optimal decision making, the agent's actions can be described by the following distribution:
                $$
                \Pr(a\vert s,\beta) = \frac{
                e^{
                \beta Q(s,a)}
                }
                {\sum_{\tilde{a}} e^{\beta Q(s,\tilde{a})}
                }
                $$
Here, $\beta$ is the rationality coefficient, where $\beta=0$ results in uniformly random (i.e., completely irrational) action selection, and $\beta\to \infty$ recovers optimal decision making under $Q(s,a)$. Open question whether we want to infer $\beta$ from observations (harder/slower) or just assume near-rational behavior. 


\clearpage

\section{Math}
Top-k
Top-p (i.e., Nucleus) sampling: top-p\% of the probability mass.
ranking / contrastive tests
could also construct goals based on distance in the embedding space (motivated by this statement from the intro read "Weight tying has an effect similar to the regularizer which forces a model to give high probability not only to the target token but also to the words close to the target in the embedding space.")
also beam search.

sanity check: compute embedding distance between different completions

idea: cluster similar completions through k-means?

potential problem: completely dissimilar goal completions may be so different bcs they dont make sense; by maximizing difference we would encourage non-sense


KnowNo: great read on answer generation in KnowNo (they just ask an LLM to generate answers for multiple choice and then add 'i dont know'

Great paper on semantic uncertainty: https://arxiv.org/pdf/2302.09664.pdf

another option to create goal locations: make another (fine-tuned?) LLM propose 'semantically diverse' goals

last option (and maybe best?; eval): 

\subsection{N-gram modelling of language}
Reminder: a common approach to modelling the likelihood of a sequence of tokens $\mathbf{z}_{<n}=z_1, . . . , z_{n-1}$ uses the following factorization:

$$
P(\mathbf{z}_{<n})=P(z_1)P(z_2|z_1)P(z_3|z_1,z_2)...
$$

My queries are token sequences of the form $\mathbf{Q}=\mathbf{N_c}+\mathbf{N_o}+\mathbf{B}$, where $\mathbf{N_c}$ is a constant part of the narration, $\mathbf{N_o}$ is an observation-dependent part of the narration, and $\mathbf{B}$ is a binding sequence. I am interested in scoring a set of possible completion series $\{\mathbf{C}_i\}$ based on how likely they are as a continuation of $\mathbf{Q}$. In other words, I am interested in a probability related to

\onecolumn

$$
P(\mathbf{N}+\mathbf{B}+\mathbf{C})
= P(\mathbf{N_c})P(\mathbf{N_o}|\mathbf{N_c})P(\mathbf{B}|\mathbf{N_c},\mathbf{N_o})P(\mathbf{C}|\mathbf{N_c},\mathbf{N_o},\mathbf{B})
$$. 

or
$$
P(\mathbf{N_c}+\mathbf{N_o}+\mathbf{B}+\mathbf{C})
= P(\mathbf{N_c})P(\mathbf{N_o}|\mathbf{N_c})P(\mathbf{B}|\mathbf{N_c},\mathbf{N_o})P(\mathbf{C}|\mathbf{N_c},\mathbf{N_o},\mathbf{B})
$$. 

Things I can compute easily: $P(N_c), P(N_o|N_c), P(B|N_c+N_o)$


The LLM gives me the probability
$$
P(\mathbf{C}|\mathbf{N_c}+\mathbf{N_o}+\mathbf{B})
$$

This can also be written as: 
$$
P(\mathbf{C}|\mathbf{N_c}+\mathbf{N_o}+\mathbf{B})
=
P(\mathbf{C}|\mathbf{N_c}+\mathbf{N_o}+\mathbf{B})
$$

Ideally, I would like to isolate the effect the observation-based narration $\mathbf{N_o}$ from that of the constant narration $\mathbf{N_c}$ and binding sequence $\mathbf{B}$. In other words, I want my score to be invariant to $\mathbf{N_c,B}$. What I tried so far is to get the score with the following normalization:

$$
s = \frac{P(\mathbf{C}|\mathbf{N_c}+\mathbf{N_o}+\mathbf{B})}{P(\mathbf{C}|\mathbf{N_c}+\mathbf{[]}+\mathbf{B})}
$$

I can compute the following from 

\subsection(Notes on LLaMA paper and general MCQA)
from the LLaMA paper:  We select the
completion with the highest likelihood given the
provided context. We follow Gao et al. (2021)
and use the likelihood normalized by the number
of characters in the completion, except for certain
datasets (OpenBookQA, BoolQ), for which we fol-
low Brown et al. (2020), and select a completion
based on the likelihood normalized by the likeli-
hood of the completion given “Answer:” as context:
P (completion|context)/P (completion|“Answer:”).

The LLaMA paper also discusses gender bias explicitly. 

observation with llama2: "Hello my name " gets completed with 'ia' instead of 'is' as the top 1 choice. If the prompt is "Hello my name" (no space at the end) the top completion is 'is'. another sign that we need to get all options by generating? another sign we need to use beam search? or spell checker? what about high percentile answers that would be spell-check transformed to one of the answers in my selection?



\subsection{Sequence generation}
Let $p_M(z_n | \mathbf{z}_{<n})$ be the probability that the language model $M$ assigns to token $z_{n}$ as a continuation for the sequence $\mathbf{z}_{<n}=z_1, . . . , z_{n-1}$. We can compute this probability as 

$$
p_M(z_{n} |\mathbf{z}_{<n})
=
\frac{
                \exp{(h_n^T e_{z_n})}
                }{
                \sum_{w\in V}\exp{(h_n^T e_{w})
                }
                }
$$

Here, $e_w$ is the output token embedding for token $w\in V$, where $V$ is the vocabulary (this is the last linear layer of the model $M$); and $h_n=h(\mathbf{z}_{<n})$ is the vector representation of context sequence~$\mathbf{z}_{<n}$. 

When generating sequences, we can adjust the desired tradeoff between diversity and coherence by scaling the next token likelihood with a softmax temperature parameter $\tau$ as shown below. Regular sampling is achieved with $\tau = 1$; low coherence (and accordingly, high levels of creativity) can be obtained by setting $\tau>1$; low levels of imagination are obtained with $\tau<1$.

$$
p_{M,\tau}(z_{n} |\mathbf{z}_{<n})
=
\frac{
                \exp{(h_n^T e_{z_n}/\tau)}
                }{
                \sum_{w\in V}\exp{(h_n^T e_{w}/\tau)
                }
                }
$$

Note: candidate sequences should always end with an 'end' token. how do we set the length of predicted sequences?
candidate generation: beam search with n beams over various values of tau




experiment ablation study: show that this uncertainty is more principled than what the KnowNo paper shoes.

\subsection{Sequence Log-Likelihood}
The log-likelihood of a sequence $\mathbf{z}_{1:n}$ can be computed as
$$
L(\mathbf{z}_{1:n})=\sum_{i=1}^n \log p_{M}(z_{i} |\mathbf{z}_{<i})
$$


\subsection{Perplexity per word}
The perplexity $PP(\mathbf{z}_{1:n})$ can be computed as
$$
PP(\mathbf{z}_{1:n})
=
\exp{
\left(-\frac{1}{n}L(\mathbf{z}_{1:n})
\right)
}
$$

\subsection{Automated goal generation}

generate a broad set of $\mathbf{g}_i$ from $\mathbf{N}+\mathbf{B}$ using high temperatue (i.e., high creativity); then score each of these goals with true temperature ($\tau=1$). compute the embedding of the resulting sequences using the same embedding used in the mapping (e.g., LSeg); and do scoring with dot product. 

Todo: make systems figure; list questions; outline approach with goal contionuations / completions (and think of an experiment that compares hand-crafted vs automatically generated goals); the goal generation and localization can also be iterative back and forth (not found in map above certain threshold? check again / generate more samples

from the LERF paper: "Comparison to LSeg in 3D: LSeg performs well on
“glass of water” since cups are in the COCO dataset, but cannot
locate an out-of-distribution query like an egg." This may be a problem if I want to use LSeg? 

noteworthy: LERF failure cases: "Failure cases: LERF struggles with identifying objects
that appear visually similar to the query: “Zucchini” also acti-
vates on other long, green-ish vegetables, and “leaf” activates on
the green plastic chair. LERF also struggles with global/spatial
reasoning, where “table” only activate on the edges of the table"

\section{Another step-by-step description}
\begin{enumerate}
    \item Generate semantic map $\mathcal{M}$
    \item Narrator generates narration $\mathbf{N}$
    \item Generate possible goals (discuss different methods to generate; open vs. closed-set; extracting from map; discuss how to get diversity; discuss how to group similar goals together to add the respective probability mass)
    \begin{itemize}
        \item one idea for goal generation: generate N samples, pick the M most likely
        \item generate N samples, pick the top-p most likely
        \item generate N samples, pick one goal. in feature space h, select the next goal sequence as the one that is most different to the previous goal sequence. iterate following something like the Gram-Schmidt process.
        evaluation metric: evaluate diversity of goals based on human rating (compare to top-k, top-p, temperature-based sampling); also compare based on coverage of the $h$ space? Can i stop generating based on coverage of the $h$ space?
        \item OPEN QUESTION: how to correct for length?
    \end{itemize}
    \item Score possible goals (discuss different scoring methods; just base don likelihood, or also based on how they were affected by the context. also discuss correction for the effect of 'sequence likelihood'
    \item translate goal description into the embedding used for the semantic map
    \item cosine similarity between features of goal description and all voxels in the semantic map
\end{enumerate}


\section{TODOS}
\begin{itemize}
    \item outline all functions i need for LLM experiments
    \item outline how i could test the goal generation on the KnowNo code and what params i would vary: temp; calibration size. how does conformal prediction change as function of calibration
    \item flesh out list from my presentation slide
    \item think through theory of answer generation and scoring in hidden params
    \item bowl in microwave example from KnowNo paper: is it the metal bowl or the plastic bowl? instead of answering with MCQA, what if we write out the answer and score it: "i will put the metal bowl into the microwave' vs 'I will put the plastic bowl into the microwave'? motivation: the MCQA approach may lose some 'world knowlegde' in the scoring when we only select A, B, C, ... for example metal and microwave = bad. broader: can we show that reducing things to MCQA options is detrimental for decision making?
    \item look at connection between embeddings and likelihoods. can I compute the likelihood of an embedding instead of a token sequence?
    \item effect of MCQA framing with finetuning vs 'story-like' framing with binding sequence and continuation
    \item take another pass at finding xx? 
    \item: idea: (mathematically) trace back which part of the context affected the robot decision in a rigorous way -> we can use this in the case where we have different trust levels in different aspects of the sensing/context! similar as in uncertainty-aware updates. 
\end{itemize}

observation: everyone seems to make up their own baselines...

what we do differently: predictive capability?


\section{System overview}
\begin{enumerate}
    
    \item Narrator
    
        \begin{itemize}
            \item Photo/video narrator
            \begin{itemize}
                \item Human detection
                \item Object detection
                \item LLaVA scene description
                \item assertion that the object 'held by the human' is close 
            \end{itemize}
            \item Apartment state narrator: time of day, appliance usage
        \end{itemize}
    
    \item Semantic map
    
\end{enumerate}


note: concept-fusion paper comes with a great demo related to 'where can I find...'; downside of their demo: they ask the LLM to rank possible locations (like many other works) after querying the map for what is available and go to the top location. instead, our scoring is more principled. 

TODO next: make list of differnet goal completion approaches

from the cartier paper (seems sketch): "We solve the
latter by generating five different answers, and selecting
the highest probability answer (as determined by the LLM)
which contains an object from the list. Empirically, we find that 5 different answers is sufficient to ensure that at least
one contains an object from the list."

TODO: think of examples with equally likely goals, either for item retrieval or human goal locations. use this example to try highlight shortcomings of various goal proposal methods. 

another option to highlight shortcoming: use method on multiple choice questions in which MULTIPLE answers can be correct! (this could be a baseline for me)

we often read LLM = world knowledge. but how do we separate world knowlegde from common patterns of speech?

"I have to go to the bathroom" vs "I have to go to the kitchen": the former is probably much more likely in language, but should not be much more likely in terms of world knowlegde.

another possible baseline: multiple choice answering where all questions are wrong (or even nonsense words). evaluate LLM confidence. evaluate whether the answers are biased towards more frequent words. for example: the best spot to sit on is 'bananas', pineapple, kumquat. or bananas on pizza, pineapple on pizza, kumquat on pizza.

questions for option generation: does it say 'unknown'? importance of adding option 'unclear'. how do you get a proper PDF? what is in the 'other group'? what happens to the answer distributions when you add 'unknown' vs 'unknown' and 'other' and 'something else'?

TODO: review and make table of how other works generate answers to LLMs


contributions:
\begin{itemize}
    \item demonstrate the utility of LLMs in predicting human intent (and goal positions) from open-set observations
    \item review and quantitatively evaluate LLM option generation methods which will find utility in robot planning and human intent prediction, as well as open-set question answering (?)
    \item present a new method to generate options
    \item present a hierarchical / pyramid approach for semantic maps / spatial language indices that achieves higher localization accuracy across object scales (specifically, it retrieves bounding boxes and center of object accurately on the map). we can achieve this by fusing at different scales and maintaining a multi-scale feature vector for each grid or pixel. useful where assemblies are distinct from individual objects example: at small scale, a pixel is part of a couch, at large scale it is part of the living room. different example: at small scale it's a hammer, at large scale it's part of a tool box). interesting example to see if it works in both cases: "fetch me the cup from the living room table" vs "fetch me the cup from the kitchen table"
\end{itemize}


\section{VLMaps paper reminder}
\url{https://arxiv.org/pdf/2210.05714.pdf}

\section{and more notes..}
nice section from the LERF paper on how to query LERF: "Often, language models like CLIP are evaluated on zero-
shot classification, where a category is selected from a list
guaranteed to include the correct category [28]. However, in
practical usage of LERF on in-the-wild scenes, an exhaus-
tive list of categories is not available. We view the open-
endedness and ambiguity of natural language as a benefit,
and propose a method to query 3D relevancy maps from the
LERF given an arbitrary text query. Querying LERF has
two parts: 1) obtaining a relevancy score for a rendered em-
bedding and 2) automatically selecting a scale s given the
prompt."


another cool example: bike pushing outdoors

cool thing about LLMs: universal use (time dependence)

take-away from discussion with Bhoram: measure for level of surprise / anomalous behaviors / events

note: idea: compare quantitatively to concept-fusoin approach with ranking responses. ranking responses should fail when two are equally likely. experiment: 'assign likelihood to each of these goals'

open-set goal queries rather than closed-set. 


and more notes: knowNo forces answer scoring into multiple choice answering, which is not appropriate in our case. this is however one way of doing things that I should discuss. the calibration step in KnowNo seems unsatisfactory. in our paper, I should highlight that the approach is calibration / training FREE! my completion generation also works for the robot control use case. 

how does the KnowNo paper achieve diversity in their answers? looks like they just achieve this with few-shot prompting, which seems a bad idea. "We can address this length bias with a simple trick. First, with
a few-shot prompt that includes possible next steps in a few scenarios (Fig. A1), the LLM generates a
set {yi} of candidate next steps (e.g., “Put plastic bowl in microwave”, “Put metal bowl in microwave”,
etc., in Fig. 1) that are semantically different. " My point: few-shot tuning with prompting is unprincipled. 

KnowNo page 3 'robots that ask for help' provides a great step by step on template for inspiration on how we can outline our work; also nce description of the 'context.'

question? how do we make sure our LLM-generated goals are affected by the right context?

\newpage
\newpage
\newpage

\section{First experiment}
\subsection{Overview}
\begin{itemize}
    \item Generate stories from a template: 
\begin{quote}

It is \{time\}.

EITHER
\begin{quote}
A human is stepping into the \{currentRoom\} from the \{previousRoom\}.
\end{quote}

OR
\begin{quote}
The human is \{sitting/standing\} in the \{currentRoom\}.
\end{quote}

The human is holding \{object/nothing\}.

FOR appliance in availableAppliances:
\begin{quote}
The \{appliance\} switched from \{previousState\} to \{currentState\} \{m\} minutes ago.
\end{quote}

\end{quote}
\item Rewrite these stories in different styles using e.g. ChatGPT (should probably be a model that is different from what we use later on)

\item Tie the story to a room layout. Work with a few vastly different layouts, i.e., one in an open office, on in an apartment without a laundry room, one in a house with multiple bathrooms, ...

\item Do a user study: show users the story and the floor plan, and ask them to select where the human will go. 

\item Evaluate the agreement between human user and our LLM predictions. 
\end{itemize}

\subsection{Questions}
Is it fine to manually craft the the sentences describing possible goals for this experiment?

\section{perplexity}
This is a great read on 'model perplexity' (which is closely related to likelihood of token) and gives background of how to deal with this for fixed length predictions: \url{https://huggingface.co/docs/transformers/perplexity}


\section{Experiments / questions}
compare the different approaches of grounding; 
see how often things are grounded in map, see how often things are true
what happens without grounding (using just completion).
will be curious to see: how do different levels of granularity affect log prob? holding a tooth brush -> likelihood of 'to the bathroom' vs. 'to the toilet in the bathroom' vs 'to the sink in the bathroom' vs 'to the shower in the bathroom'
what happens with the likelihood of predictions when we add the options 'unknown', 'random', 'A or B' as completion vs. if these options are not available? What about the cost of 'no completion'
test with somewhat unusual placements, like "the laundry machine in the kitchen" or very similar goals like 'holding a toothbrush; the sink in the kitchen vs the sink in the bathroom'
what's the change in performance for text completion vs boiling things down to multiple choice directly vs multiple choice after chain-of-thought prompting?
another idea: what happens if the human wants to brush their teeth but the bathroom is occupied? will the LLM say the human is gpoing to the sink?


\section{Problem definition}
\noindent
\textbf{Given}
\begin{enumerate}
    \item A floor plan with semantic information (can be a visual language map or \textit{VLMap} as presented in \cite{huang2022visual} or a map with localized language labels) $\mathcal{M} \in \mathbb{R}^{L\times W \times C}$, where $L$,$W$ are the length and width of the grid representing the top-down floor plan, and $C$ is the dimension of the feature vector encoding semantic information for each grid cell of the floor plan.
    \item An observation the human and the apartment state, resulting in a set of $n$ features $\mathbf{x}=(x_1,...,x_n)$ describing the state of the human and the apartment.
\end{enumerate}

\noindent
\textbf{Aim 1: Inference of likely human goal positions} We have a grid of possible goal cells of size $L \times W$ and want to infer the likelihood $\mathcal{G} \in \mathbb{R}^{L \times W}$ that a given cell is the goal position. Having no knowledge about the human intent, each element of $\mathcal{G}$ is a goal with equal probability $\frac{1}{LW}$. 

\noindent
\textbf{Aim 2: Forecasting of human trajectory} We want to predict the future human trajectory/position for the next $T$ steps. We can either predict the coordinates $s_{t:t+T}$ of the human's Center of Mass (CoM) or predict the likelihood of occupancy for the next $T$ steps on an occupancy grid $\mathcal{O}_{t:t+T} \in \mathbb{R}^{L\times W}$

\noindent
\textbf{Aim 3: Human-aware, safe and reactive planning} Account for the predicted human trajectories and the obstacles in the world and incorporate it all into RAMP.

\noindent
\textbf{Approach}
\begin{enumerate}
    \item Extract features $\mathbf{x}$ ...
    \begin{itemize}
        \item ... from camera: \begin{itemize}
            \item detect and crop human
            \item possibly detect / crop human hands to find tools
            \item detect items / tools held by the human
            \item if possible, detect information about clothing
        \end{itemize}
        \item ... from camera or other sensors: 
            \begin{itemize}
                \item human position on the floor plan
                \item possibly past trajectory
            \end{itemize}
        \item ... from smart home: 
            \begin{itemize}
                \item current appliance state (e.g., washing machine on/off)
                \item last state transition (e.g., finished running)
                \item time since last state transition
            \end{itemize}
    \end{itemize}
    \item Construct LLM query: 
        \begin{itemize}
            \item Describe apartment layout in natural language (connectivity of rooms, key objects and appliances in each room)
            \item The local time is 13:00.
            \item Appliances (dish washer or laundry machine): if appliance finished running within the last $m$ minutes, state that "The [appliance] stopped running $m$ minutes ago."
            \item Describe the human: what objects / tools are they holding, what are they wearing?
            \item "Where are they most likely going next?"
            \item "What other scenarios can you think of?"
            \item Optionally: provide the LLM with a set of available goals to choose from (goals parsed from $\mathcal{M}$)
        \end{itemize}
    \item Receive LLM answer and parse it to update $\mathcal{G}_{LMM}$
        \begin{itemize}
            \item either hard code this step, or compare similarity of predicted goal in text form with the feature vector on $\mathcal{M}$
        \end{itemize}
    \item Optionally: Bayesian update to ensure consistency between the LLM-predicted goal and the goal map $\mathcal{G}_F$ that would be inferred from the past trajectory with a motion-based filter (e.g., Kalman filter) 
        $$
            \mathcal{G}=
            \frac{w_1\mathcal{G}_{LMM}+w_2\mathcal{G}_{F}}
            {\sum_i w_i}
        $$  
    \item Get likely human path from goal map $\mathcal{G}$ and traversability map $\mathcal{T} \in \mathbb{R}^{L\times W}$
        \begin{itemize}
            \item We can get the 2D traversability map $\mathcal{T}$ from $\mathcal{M}$ by projecting $C$ to one dimension with a binary score that indicates whether the underlying area is traversable or not. Alternatively, we could project $C$ to a continuous traversing cost score that reflects the a priori likelihood of the human to traverse a certain area (e.g., a grid cell containing wall features in $C$ should have a traversability of $0$; tables should result in similarly low traversability; chairs and easily movable obstacles should have a higher traversability; and open space should be easily traversable. 
            \item We can construct an estimate of the human's utility or state-action value function $\hat{Q}(s,a)$ from $\mathcal{G}$ and $\mathcal{T}$.
            \item Then, the trajectory can be obtained under the assumption that the human is an agent taking action $a_t$ with the goal to maximize its utility. A perfectly rational agent would take the action $a_*=\arg\max_a Q(s,a)$. Following a noisy-rationality decision model (e.g., \cite{ziebart2008maximum}, but also applied and discussed in depth in \cite{fisac2018probabilistically}) instead of optimal decision making, the agent's actions can be described by the following distribution:
                $$
                \Pr(a\vert s,\beta) = \frac{
                e^{
                \beta Q(s,a)}
                }
                {\sum_{\tilde{a}} e^{\beta Q(s,\tilde{a})}
                }
                $$
            Here, $\beta$ is the rationality coefficient, where $\beta=0$ results in uniformly random (i.e., completely irrational) action selection, and $\beta\to \infty$ recovers optimal decision making under $Q(s,a)$.
        \end{itemize}
    \item Integration with RAMP:
    \begin{itemize}
        \item From likely human path, get a cost map that encourages the robot to avoid the human path
        \item Do RAMP with human-aware cost map
    \end{itemize}

\end{enumerate}



\section{Formal CoM trajectory prediction}
Let $s_t=(x_t,y_t)$ be the position of a human's CoM at time $t$. Our goal is to predict the next $T$ positions from the previous positions. Alternatively, we could consider all joint angle positions and velocities as part of our state (in addition to CoM). 

We can easily extend this to multiple human agents in the scene, with $s_t^i$ representing the position of agent $i$ and $s_t=\{s_t^1,...,s_t^M\}$ being the full state of the scene with all $M$ agents. We can model this system as a Hidden Markov Model (HMM) with observable states $s_t$ and hidden states $h_t$ that affect the next state. 

One common way to solve the human trajectory forecasting problem relies on an encoder-decoder neural network architecture (e.g., as in \cite{liu2021social}), where an encoder network $f$ is used to extract an approximation/estimate of the hidden state $\hat{h}_t$, and a decoder network $g$ predicts/rolls out future trajectories based on $\hat{h}_t$.

Alternatively, the trajectory can be obtained under the assumption that the human is an agent taking action $a_t$ with the goal to maximize its utility. A perfectly rational agent would take the action $a_*=\arg\max_a Q(s,a)$. Following a noisy-rationality decision model (e.g., \cite{ziebart2008maximum}, but also applied and discussed in depth in \cite{fisac2018probabilistically}) instead of optimal decision making, the agent's actions can be described by the following distribution:

$$
\Pr(a\vert s,\beta) = \frac{
e^{
\beta Q(s,a)}
}
{\sum_{\tilde{a}} e^{\beta Q(s,\tilde{a})}
}
$$

Here, $\beta$ is the rationality coefficient, where $\beta=0$ results in uniformly random (i.e., completely irrational) action selection, and $\beta\to \infty$ recovers optimal decision making under $Q(s,a)$.

Old-school baseline: Kalman filter / conservation of momentum


\section{Tasks}
\subsection{(Zero-shot) human goal inference}
where will the human go?

datasets:

baselines:

\subsection{Next action/activity prediction}
given a sequence of past actions/activities, what is the likely next action?

the effect of temporal context on action recognition is studied in the paper "With a Little Help from my Temporal Context: Multimodal Egocentric Action Recognition" \url{https://arxiv.org/pdf/2111.01024.pdf}: "capitalise on the action’s temporal context and propose a method that learns to attend to surrounding actions in order to improve recognition performance. To incorporate the temporal context, we propose a transformer-based multimodal model that ingests video and audio as input modalities, with an explicit language model providing action sequence context to enhance the predictions. (...) audio-visual model utilises two separate summary embeddings to attend to the action (i.e. verb) class and the object (i.e., noun) class. This allows the model to attend independently to the temporal context of verbs
vs objects. For example, the object is likely to be the same in neighbouring actions while the possible sequences of verbs can be independent of objects (e.g. ‘take’ $\to$ ‘put’). Each summary embedding uses a different learnt classification token, and the classifier predicts a verb and a noun from the summary embeddings. (...) We use the language model to improve the predictions of the audio-visual transformer by filtering out improbable sequences. (...) We train this model independently from the audio-visual transformer. Specifically, given a sequence of actions Y = (...), we randomly mask any action Yj and train the model to predict it. For example, an input sequence to the model (for w = 5) would be (‘turn on tap’, ‘wash hands’, <MASK>, ‘pick up towel’, ‘dry hands’). " overall, this paper is a very good resource for formalism. I do believe that this paper uses training (\textbf{TODO: double check}). If yes, it would be nice to show comparable performance using zero shot approach. 

datasets:

baselines:

\subsection{object pairing prediction}
milk jug will be moved (by the human) to the cup

\subsection{object home base position}
the cup belongs into the cupboard or dishwasher


\section{Random notes on research questions and vague ideas}
\begin{itemize}

\item idea: the zero shot ability of LLMs is particularly relevant when encountering unexpected behaviors (which robots WILL encounter). to use this in a robotic context, we need the ability to parse the LLM's understanding of what is happening to a language that is actionable for the robot. what could this be? relevant dataset with unexpected events: \url{https://dl.acm.org/doi/10.1145/3371382.3378270}

\item possible experiment: ablation study: same query as with the cup, but human holds a random object that should have nothing to with possible targets.

\item predicting 'attractor regions' - i.e., likely goals. a given item/object has some connection to several attractor regions. how likely the attraction is depends on the human's trajectory, time of day, apartment information, ...

\item when computing the log-likelihood completion cost for completions with the various goals, do we need to discuss how to account for the cost of 'no completion'?

\item train/fine-tune with loss to enforce consistency between meaning of verbal description / prediction of an LLM of what will happen and scene dynamics. LLM query: "what happens when a cup moves over the edge of a table." LLM answer: "When a cup moves over the edge of a table, it will typically fall downward due to the force of gravity acting on it. The specific outcome will depend on various factors such as the cup's initial velocity, angle of movement, the shape of the cup, the table's height, and other environmental conditions.

If the cup's center of mass remains within the base of support (i.e., the part of the cup that is still on the table) as it moves over the edge, it may continue to stay upright. However, if the cup tilts or if its center of mass moves beyond the base of support, it will lose stability and topple over.

As the cup falls, it will follow a parabolic trajectory due to the combined effects of gravity and any initial velocity it had. The cup may collide with objects on its way down or break upon impact with the floor, depending on the cup's material and the force of the fall.

It's important to note that this explanation assumes idealized conditions and neglects any potential external factors, such as air resistance or other forces acting on the cup, which may affect its motion."

\item novelty of our paper most likely comes from the connection between LLM inference and trajectories in space (trajectories of the human CoM, its limbs i.e. hands, and of objects). another source of novelty: accounting for time of day (some work has shown time of day is a good predictor for activities, e.g. the german time use study. try to show quantitatively that LLMs are aware of how time and activity are related as a sub-result, then put everything together). and another source of novelty: apartment state information. sure, we can predict 'wash the aubergine', but what does this actually mean in terms of how human and object poses change?

\item downside of VLmaps as stated in their paper: "They
also cannot resolve object ambiguities during landmark indexing
when the scene is cluttered with similar objects. In future work, we
plan to improve VLMaps with better visual language models and
to extend it to scenes with dynamic objects and moving humans."

\item another idea: adapt the narration based on whether a certain detail affects the distribution of the predicted next actions, or find out which piece of the narration was how important in the resulting intent prediction

\item idea epic kitchens action anticipation challenge: maintain a state of last touched items or items in near proximity or items generally nearby; explicitly maintain how long the lats action has been going on, and maintain a list of last actions

\item relevant papers: concept fusion paper and openscene paper. concept fusion has reasonably good demo code available online.

\item demo vision: robot is executing a pick and place task with many objects (lots of back and forth) as a human walks into the scene holding a coffee mug. the robot adjusts his task ordering to account for the human walking by.

\item distinction from prior works: \begin{itemize}
    \item Andrea Bajcsy et al.: great work on probabilistically safe planning under the following strong assumption: "We assume that the robot has a suitable human reward
function, either learned offline from prior human demonstrations or otherwise encoded by the system designers." they assume that the goal position is known. 
\item lots of semantic maps exist: VLMap, openscene, 
\item 
\end{itemize}

\item possible areas for LLMs to shine: where training data is sparse (ie zero shot), or where number of predicted classes is infinite (but then i need a way to extract actionable insights from the LLM prediction), or where the info obtained is very poor in information (e.g., no video available).

\item interesting observation. Query: "an open office is connected to an exit door, a bathroom, and a kitchenette. It is 11am. Moritz, an employee at the office, gets up from his desk. where is he most likely to go? give a one-word answer." the answer goes back and forth between 'kitchenette' and 'bathroom' - consider a sampling-based approach (i.e., query the model N times and count the answer frequencies). Interesting experiment: visualize how the answer distribution is affected by time of day, then compare it to see whether it is consistent with some time use studies from the US. 

\item brief blog post on using the logit bias argument in chatgpt: \url{https://help.openai.com/en/articles/5247780-using-logit-bias-to-define-token-probability}

\item instead of prompting with 'unknown' or 'random' as an answer option, marginalize over all tokens that translate to 'random' unknown, either, i dont know, .... how to do this in a principled way? there should be some latent space representation in which these similar words are close. how can I access them? also, similarly, we could marginalize over 'right/kitchenette' and 'left/bathroom' tokens in the case where we have to decide between the left bathroom door and the right kitchenette door. idea: get group of tokens over which we marginalize from the semantic map. an area from the semantic map has some tokenized representation for each pixel (or voxel) we can use this to automate the possible goals. this way, all suggested target goals are always available in the scene. i know the cup belongs to the cupboard, but if there is no cupboard in the area, they are likely trying to put the cupboard somewhere else. we can query a specific area on the map for possible goals based on the past trajectory and a simple motion-based forecasting model. 

\item link to VLMaps code lab

\item another idea: this can also allow us to localize the human if we know activities they are doing without seeing them (for example, the stove is on -> they are most likely cooking -> they are likely in the kitchen)


\item discussion with Volkan about two examples of multi-step reasoning: 
\begin{itemize}
    \item "I grabbed the coke from the fridge and brought it to the study and left it there. where is the coke?" also consider changing the last sentence to 'where is it'? what is the answer of the model? 
    \item chatgpt older model: beam search. todo moritz: re-read the paper to understand their inference
    \item "I could not put the hammer into the box because it was too big. ... what was too big?" unclear whether it was the box or the hammer to the model. how can we resolve this disambiguity?
    \item possible idea: likelihood of next tokens may be distributed almost evenly between two (or N) possible answers, but the LLM choses one that may be wrong. we can use traditional robotics / path planning / motion prediction / logic / geometry / or even self consistency ! to resolve this problem
    \item related idea: resolving the disambiguity between possible goal positions with the past trajectory of the human
    \item from discussion with Volkan: he said chatgpt uses beam search, but I think this post has some people/commenters who disagree with that assessment. \url{https://www.reddit.com/r/LocalLLaMA/comments/13zlbt6/chatgpt_uses_beam_search_your_local_models_use/}
\end{itemize}
\item action anticipation in the epic kitchens dataset is pretty much what we want to do. \url{https://epic-kitchens.github.io/2023#challenge-action-anticipation}

\item another idea: use some human walking tracking/prediction dataset and forecast human trajectories like in the social NCE socially aware motion representations paper but extend the concept to 'environment-aware motion representations' by taking into account the spatially resolved CLIP embeddings.  

\item question: can we use chain of thought prompting with few-shot training with examples that have nothing to do with human actions to motivate the LLM to do good chain-of-thought reasoning on human next step predictions? 

\item another question related to chain-of-thought prompting: can we use labels from action sequences for prompting with sequences / long-horizon predictions/anticipation?

\item another possible pitch: each of the individual tasks (like predicting where employee Moritz goes as a function of the time) is doable / easy-ish to train iwth data. but doing all of these types of tasks with zero shot learning with varying input info is a unique strength of the LLM-based approach. 

\item note: saycan paper figure 1 has very different outputs between the different LLMs. this was also a problem I observed with my trials. how can I ground them in reality? traditional traj planning for the human. 'avoid other humans' 

\item todo: craft more LLM example queries for the 'object-goal pairing/attractor regions' concept

\item attractor concept: doorways also are an attractor for humans. 

\item possible argument for why we should use LLM priors: smoother collaboration in the beginning, and maybe the ability to avoid catastrophic failures.

\item longer-term project: learn full joint or mesh forecasting model and condition the prediction on narration of the previous video and an LLM with 'what will happen next'. needs a dataset with realistic tasks and skeleton or mesh annotations of humans.

\item todo: for all the datasets, note whether they were taken 'in the wild' or in artificial settings or by actors or... 

\item idea for the TREK-150 Object Tracking data (paper at \url{https://arxiv.org/pdf/2209.13502.pdf}), get the activity (e.g., pour, put, place, ...) and translate them into trajectories in 3D. pour A into B means 'content A goes from container of A into B'

\item possible a strong criticism of the KnowNo paper: if it works so well with 'probabilistic guarantees', why do you have to force it to use multiple choice questions? todo mo: doesnt that ruin a lot of the distribution? read the paper again and pay careful attention to this

\item What does it mean to predict human intent?
    \begin{itemize}
        \item Predict future center of mass (CoM)
        \item Predict future joint poses
        \item Predict future hand positions
        \item Predict the next object the human interacts with
        \item Predict where the human will move the object they are interacting with
        \item Predict the next action ('action anticipation' in EPIC Kitchens-100)
        \item What do future frames look like?
        \item Predict desired human goals (and then derive the path from that prediction); predict likelihood over human goal spots.
        \item related stuff from \url{https://arxiv.org/pdf/2110.07058.pdf}: "Relation to existing tasks Predicting future events from egocentric vision has increasing interest [191]. Previous work considers future localization [113, 120, 174, 230], action anticipation [76, 77, 86, 118, 127, 219], next active object prediction [20,74], future event prediction [149,167], and future frame prediction [145, 146, 153, 215, 218, 227]. Whereas past work relies on different benchmarks and task definitions, we propose a unified benchmark to assess progress in the field." 
    \end{itemize}

\item another idea: query the LLM in a more open-ended way, like "what are some places where a human might want to place an [object they hold]?" - then query the VLMap for places. 

\item looks like chat completion can create log probabilities of the most likely returned tokens. the best\_of parameter also seems relevant for sampling. see \url{https://platform.openai.com/docs/api-reference/completions/create}

\item how can i get guarantees for LLMs / LLM predictions? what does self-consistency mean in the context of human motion prediction? maybe it means aligning short-term predictions from past motion with long-term goal inference?

\item notes from meeting on june 27 2023: let's get the logits directly for next token likelihood instead of shitty sampling. this should more accurately model the distribution of

\item to check: are we just sampling the proximity in latent space between 'coffee mug' and kitchen? Volkan brought up this question. if yes, is this a problem, or is it fine?

\item ideally, generate the query from the semantic map directly, rather than manually prescribing goals and then matching them to the map.

\item slightly different idea: on pure pedestrian locomotion dataset, use VLMaps/CLIP to learn features that push humans away and features that attract humans.

\item another idea: look at active learning of behavior over time; ideally show that by starting with info from LLM i can learn better/faster/SAFER than without llm (on existing dataset with learning goal inference as we move through the dataset

\item great formulation on how to correct robot paths with natural language feedback (e.g., go slower) in this paper Jinwook sent: \url{https://www.roboticsproceedings.org/rss18/p065.pdf}

\item paper plan: zero shot inference of goal positions based on: (1) time of day, (2) objects the human is carrying, (3) apartment features (e.g., all the lights where just turned off)

\item another potential pitch: the LMM approach is useful for sensorized homes (like in the MIT activity recognition dataset) and (narrated) video data, when both modealities are available, but also when only one of the modalities is available. 


\item condition the mesh prediction in an approach similar to \url{Humans in 4D: Reconstructing and Tracking Humans with Transformers} on an LLM with the query 'last actions where xyz (from video narrator). what is the human likely doing next'?


\item different approach idea: can we just use LLMs for pretraining in next-action / next-activity prediction tasks, similar to \url{https://arxiv.org/pdf/2212.04501.pdf} but use their inherent embedding to better predict what's next in action space? justification: inherently, they have a latent space representation somewhere that understands what's next. potentially also prompt the right latent space with 'what will happen next' always added?


\item using LLMs plus VLMaps plus object detection to infer pairs of "object A will likely go to B" or "A belongs to B". maybe combine this with a memory of recently seen things? useful for kitchen cleanup but also watching robot assembly. for example, predict that the screw driver goes to the screw, nail to hammer, ..., could formulate it as attraction/repulsion potentials? use which entities are connected / grounded to each other? in the milk jug example, the mug is grounded to the counter with high likelihood, and the milk is grounded to the hand

    \item Using LLMs to make the connection between tools and location / occupancy likelihood: The human is holding a drill $\to$ it is unlikely that they are taking a shower or sitting down in front of the TV. the human is holding a knife in the kitchen $\to$ it is unlikely that they are going to walk into the living room. they are most likely going to stay in the preparation area.


\item idea for evaluation: amazon turk: given an image (or verbal description) of a human, where in the map are they going? todo: ask Volkan and team members how convincing this is.


\item possible area of research: using LLMs connected to object affordance prediction. An old starting point for literature search is \cite{koppula2013learning}.

\item showing that insights trained and evaluated on one activities of daily living dataset dont transfer well across datasets, but if we use LLMs as a source/prior for knowledge, it transfers well.

\item could also show that incorporating LLM knowledge helps with transferring from simulation to real-world, and compare to the GTA dataset. 

\item can we use sitcom video with reconstructed floor plans for evaluation?

\item could also try look at collaborative assembly tasks / videos / datasets to demo the concept?

\item show zero shot learning, i.e., show that we don't need any learning

\item LLMs can also be used to indicate which object the human most likely wants next

\item todo find out: how do variations in the query affect the predicted goal. for example, 'the human looks at the table' vs things that should not matter, e.g. the human looks at his phone. Does adding irrelevant information to the LLM query affect the prediction? how does the sentence 'the appliance finished running $m$ minutes ago' affect the query if we increase $m$ to days?

\item focus on zero shot intent and connection between objects / tools and behaviors. What does it mean if a human holds a jug? the LLM knows. :P

\item Show that we need far less data for training activity recognition (or next activity prediction) by incorporating LLMs. Given a sequence of actions, what is the likely next action? Example: (1) put a mug on a counter, (2) open the fridge, (3) grab a jug of liquid from the fridge, what is the likely next action? A: pouring liquid into the mug. What does this mean for the human movement / occupancy grid?

another idea: can we use LLMs to predict degrees of freedom of objects or predict how humans are likely to move objects around?
\item another important idea: how can we force the video narrator to mention details that are relevant, like what items the human is holding?

\item the KnowNo paper \url{https://arxiv.org/pdf/2307.01928.pdf} has a good justification for why we should use Multiple choice framing to evaluate uncertainty in their section A1

\end{itemize}



\section{Random notes again}
from \url{https://www.philkr.net/media/zhao2022learning.pdf}: "Following the formulation of factorized probabilities in language models [5], we model the visually conditioned text likelihood as follows: (...)" provides a possible framing for our approach. 

what we want is to predict the human's next position/action (or next poses in the case of granular pose forecasting) conditioned on: (1) visual evidence, (2) knowledge about human motion model, (3) LLM narration (possibly queried with 'what will happen next?').

\section{other notes}
other ntoes: Contribution 1: tying the LLMs prediction of what the human will do next to what is available in their environment $E$. the most natural place for a cup is likely in the cupboard, but if there is no cupboard nearby, that's not the humans intention

\section{Contributions}
Contribution 1: LLMs grounded in reality

Contribution 2: combining the above with trajectory-based goal inference

Contribution 3: planning to avoid the human at different levels of granularity (by room, by trajectory / non-collision). show that this is much faster than always worrying about the trajectory



\section{More relevant papers}


I started a collection of 'traditional' literature on human intent prediction and motion forecasting here: \url{https://docs.google.com/spreadsheets/d/1sjq4m4uJu3U5lnQLdU1J6qlwgAUhiZAc8zuwxzSZjws/edit?usp=sharing}.



==> old_notes/other_notes.tex <==

\section{Reminder: image classification, formally}
Given: a set of $K$ class labels $Y$, a set of samples $X$, and a sample image $x$. Goal: get predicted class $\hat{y}$.

Classification (frequentist): $\hat{y}=f(x)$

Bayesian classification (more info at \url{https://en.wikipedia.org/wiki/Naive_Bayes_classifier}): ${\hat {y}}=\operatorname{\arg \max }_{{y}}\Pr(Y=y\vert X=x)$. Note that we can also frame our task as classifying based on a set of $n$ features $\mathbf{x}=(x_1,...,x_n)$ that are extracted from the image $x$, meaning that our goal is to find $${\displaystyle \Pr(y_{k}\mid \mathbf {x} )={\frac {\Pr(y_{k}) \Pr(\mathbf {x} \mid y_{k})}{\Pr(\mathbf {x} )}}\,}$$ and then get the predicted class as $\hat{y}=\operatorname{\arg \max }_{{y_k}}\Pr(y_{k}\vert\mathbf{x})$.

Note: deep neural network classifiers tend to be overly confident and poorly calibrated, meaning that the scores they return are not true class probabilities. Calibration is possible, e.g., using Platt scaling \cite{pmlr-v70-guo17a}.


\section{Formal task definitions}

\subsection{Next room occupancy (NR)}
Given: a set of $K$ rooms $Y$ (and, possibly, a graph $G$ representing how the rooms are connected). Given the state of the world as a feature vector $\mathbf{x}$, to which room is the human going next?

Traditional approaches: state transition matrix or Hidden Markov Model (HMM)

Features describing the state of the world can include: 
\begin{itemize}
    \item Human's center of mass (CoM) trajectory history
    \item Human pose history
    \item Human gaze
    \item State of apartment and appliances: time of day, temperature and humidity, air quality, light settings, laundry (e.g., off, running, done)
    \item Information about items / tools the human is holding
    \item Information about the human's appearance (wearing a towel)
\end{itemize}


We want to infer likely human goal positions. We have a grid of possible human goal cells $\mathcal{G} \in \mathbb{R}^{L \times W}$. Having no knowledge about the human intent, each element of $\mathcal{G}$ is a goal with equal probability $\frac{1}{LW}$. 

We also want to extract likely paths from the current position to the goal that accounts for obstacles. We can get 2D obstacles from $\mathcal{M} \in \mathbb{R}^{L\times W \times C}$, by projecting $C$ to one dimension with a binary score that indicates whether the underlying area is traversable or not. alternatively, we could project $C$ to a continuous traversing cost score that reflects the likelihood of the human to traverse a certain area.

$$
\mathcal{G}=
\frac{w_0\mathcal{G}_{LMM}+w_1\mathcal{G}_{F}}
{\sum w_i}
$$


\subsection{Goal inference (GI)}
Same as next room occupancy problem, but with higher granularity. Can either be framed as predicting the likely goal from a discrete set of goal locations or as a heat map over a discretized floor map that shows likely target positions.

From a set of possible goal states/intentions/objectives/aims/tasks/target positions $S_g$, infer the most likely goal state $s_g$ (or, alternatively in the Bayesian setting, get the probability $\Pr(S_g=s_g\vert O=o)$) given an observation of the environment $o$.

Alternatively, this can be framed as inferring the human's utility or state-action value function $Q(s,a)$.

Specifically, try to connect a human's tools or appearance, as well as timing information, to likely goal positions.





\subsection{CoM trajectory prediction}
Let $s_t=(x_t,y_t)$ be the position of a human's CoM at time $t$. Our goal is to predict the next $T$ positions from the previous positions. Alternatively, we could consider all joint angle positions and velocities as part of our state (in addition to CoM). 

We can easily extend this to multiple human agents in the scene, with $s_t^i$ representing the position of agent $i$ and $s_t=\{s_t^1,...,s_t^M\}$ being the full state of the scene with all $M$ agents. We can model this system as a Hidden Markov Model (HMM) with observable states $s_t$ and hidden states $h_t$ that affect the next state. 

One common way to solve the human trajectory forecasting problem relies on an encoder-decoder neural network architecture (e.g., as in \cite{liu2021social}), where an encoder network $f$ is used to extract an approximation/estimate of the hidden state $\hat{h}_t$, and a decoder network $g$ predicts/rolls out future trajectories based on $\hat{h}_t$.

Alternatively, the trajectory can be obtained under the assumption that the human is an agent taking action $a_t$ with the goal to maximize its utility. A perfectly rational agent would take the action $a_*=\arg\max_a Q(s,a)$. Following a noisy-rationality decision model (e.g., \cite{ziebart2008maximum}, but also applied and discussed in depth in \cite) instead of optimal decision making, the agent's actions can be described by the following distribution:

$$
\Pr(a\vert s,\beta) = \frac{
e^{
\beta Q(s,a)}
}
{\sum_{\tilde{a}} e^{\beta Q(s,\tilde{a})}
}
$$

Here, $\beta$ is the rationality coefficient, where $\beta=0$ results in uniformly random (i.e., completely irrational) action selection, and $\beta\to \infty$ recovers optimal decision making under $Q(s,a)$.

Old-school baseline: Kalman filter / conservation of momentum

\subsection{Full pose prediction}
We can either represent the human pose as a series of joint coordinates in 3D, or by joint angles. 

\subsection{Activity detection}

\subsection{Next action prediction (NA)}
Given a sequence of actions, what is the likely next action?


Example: (1) put a mug on a counter, (2) open the fridge, (3) grab a jug of liquid from the fridge, what is the likely next action?



\subsection{more ideas}
Using LLMs to make the connection between tools and location / occupancy likelihood: The human is holding a drill $\to$ it is unlikely that they are taking a shower or sitting down in front of the TV. the human is holding a knife in the kitchen $\to$ it is unlikely that they are going to walk into the living room. they are most likely going to stay in the preparation area.

make occupancy heatmap / goal heatmap. no priors $\to$ random occupancy distribution

possible area of research: using LLMs connected to object affordance prediction. An old starting point for literature search is \cite{koppula2013learning}.

another idea: showing that insights trained and evaluated on one activities of daily living dataset dont transfer well across datasets, but if we use LLMs as a source/prior for knowledge, it transfers well.

could also show that this transfer helps with transferring form simulation to real-world, and compare to the GTA dataset. 

could also try look at collaborative assembly tasks / videos / datasets to demo the concept?

maybe we can combine it with VLMaps for zero shot learning, i.e., show that we don't need any learning

LLMs can also be used to indicate which object the human most likely wants next

todo find out: how do variations in the query affect the predicted goal. for example, 'the human looks at the table' vs things that should not matter, e.g. the human looks at his phone. Does adding irrelevant information to the LLM query affect the prediction? how does the sentence 'the appliance finished running $m$ minutes ago' affect the query if we increase $m$ to days?

thought: motion-based trajectory prediction when walking to a door: the forecast should open up to 'anywhere in the kitchen' after going through the kitchen door. 

focus on zero shot intent and connection between objects / tools and behaviors. What does it mean if a human holds a jug? the LLM knows. :P

